Faster and More Robust Mesh-based Algorithms for Obstacle k-Nearest Neighbour

We are interested in the problem of finding $k$ nearest neighbours in the plane and in the presence of polygonal obstacles ($\textit{OkNN}$). Widely used algorithms for OkNN are based on incremental visibility graphs, which means they require costly and online visibility checking and have worst-case quadratic running time. Recently $\mathbf{Polyanya}$, a fast point-to-point pathfinding algorithm was proposed which avoids the disadvantages of visibility graphs by searching over an alternative data structure known as a navigation mesh. Previously, we adapted $\mathbf{Polyanya}$ to multi-target scenarios by developing two specialised heuristic functions: the $\mathbf{Interval heuristic}$ $h_v$ and the $\mathbf{Target heuristic}$ $h_t$. Though these methods outperform visibility graph algorithms by orders of magnitude in all our experiments they are not robust: $h_v$ expands many redundant nodes when the set of neighbours is small while $h_t$ performs poorly when the set of neighbours is large. In this paper, we propose new algorithms and heuristics for OkNN which perform well regardless of neighbour density.

==> src/heuristic.tex <==
\coordinate (a) at (2, 5);
\coordinate (b) at (5, 2);
\coordinate (r) at (2, 3);
\coordinate (t) at (5, 4);
\coordinate (t2) at (2, 6);
\coordinate (t3) at (3, 2);
\coordinate (q) at (1, 1);

\newcommand{\nodelabel}[2] {
    \node[fill,circle,scale=0.2,label=#2:$#1$,color=red] at (#1) {$#1$};
}

\newcommand{\drawST}[2] {
    \node[fill,circle,scale=0.2,label=#2:$#1$,color=blue] at (#1) {$#1$};
}

\newcommand{\snode}{
    \draw [gray] (a)--(b);
    \drawST{q}{right}
    \drawST{t}{above}
    \nodelabel{r}{below}
    \nodelabel{a}{above}
    \nodelabel{b}{above}
}

\newcommand{\gvalue}{
    \draw [->,black, very thick] (q.north) to [out=30,in=150] (r.north);
}

\newcommand{\hvalue}{
    \draw[black,dashed,very thick] (r)--(t);
}

\newcommand{\hivalue}{
    \draw [gray] (a)--(b);
    \drawST{q}{right}
    \nodelabel{r}{below}
    \nodelabel{a}{above}
    \nodelabel{b}{above}
    \gvalue
    \draw[black,dashed,very thick] (r)--($(a)!(r)!(b)$);
}


==> src/targeth.tex <==
\definecolor{zzwwqq}{rgb}{0.6,0.4,0.}
\definecolor{ccqqqq}{rgb}{0.8,0.,0.}
\definecolor{qqwwtt}{rgb}{0.,0.4,0.2}
\definecolor{qqzzqq}{rgb}{0.,0.6,0.}
\definecolor{ududff}{rgb}{0.30196078431372547,0.30196078431372547,1.}
\coordinate (a) at (2.5, 2.5);
\coordinate (b) at (3.5, 2.5);
\coordinate (c) at (3.2, 2.5);
\coordinate (r) at (3, 2);
\coordinate (r') at (3, 3);
\coordinate (t1) at (1.63, 2.28);
\coordinate (t2) at (1.33, 3);
\coordinate (t3) at (2.5, 3);
\coordinate (t4) at (3.5, 3.5);
\coordinate (t5) at (4.18, 2.82);
\coordinate (t6) at (4.52, 2.27);
\coordinate (t7) at (3.5, 1.7);
\coordinate (t8) at (2.5, 1.5);

\newcommand{\nodelabel}[2] {
    \node[fill,circle,scale=0.25,label=#2:$#1$,color=ududff] at (#1) {$#1$};
}

%\draw [line width=2.pt,dash pattern=on 2pt off 2pt,domain=-0.7621281650478093:3.0] plot(\x,{(-2.5--0.5*\x)/-0.5});
%\draw [line width=2.pt,dash pattern=on 2pt off 2pt,domain=3.0:5.571634219160852] plot(\x,{(-0.5--0.5*\x)/0.5});
%\draw [line width=2.pt,dash pattern=on 2pt off 2pt,domain=-0.7621281650478093:3.0] plot(\x,{(-0.-0.5*\x)/-0.5});
%\draw [line width=2.pt,dash pattern=on 2pt off 2pt,domain=3.0:5.571634219160852] plot(\x,{(--3.-0.5*\x)/0.5});

\newcommand{\drawra}{
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=1.0:3.0] plot(\x,{(-2.5--0.5*\x)/-0.5});
}
\newcommand{\drawrb}{
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=3.0:5.0] plot(\x,{(-0.5--0.5*\x)/0.5});
}
\newcommand{\drawrpa}{
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=1.0:3.0] plot(\x,{(-0.-0.5*\x)/-0.5});
}
\newcommand{\drawrpb}{
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=3.0:5.0] plot(\x,{(--3.-0.5*\x)/0.5});
}

\newcommand{\areaA}{
  \fill[line width=2.pt,color=ccqqqq,fill=ccqqqq,fill opacity=0.1] (2.5,2.5) -- (1.,4.) -- (1.,2.5) -- cycle;
  \draw[color=ccqqqq] (1.24, 3.3) node {$areaA$};
}

\newcommand{\areaAp}{
  \fill[line width=2.pt,color=ccqqqq,fill=ccqqqq,fill opacity=0.1] (1.,2.5) -- (1.,1.) -- (2.5,2.5) -- cycle;
  \draw[color=ccqqqq] (1.25, 2) node {$areaA'$};
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=1.0:3.0] plot(\x,{(-2.5--0.5*\x)/-0.5});
}

\newcommand{\areaB}{
  \fill[line width=2.pt,color=zzwwqq,fill=zzwwqq,fill opacity=0.1] (3.5,2.5) -- (5.,4.) -- (5.,2.5) -- cycle;
  \draw[color=zzwwqq] (4.6,3.28) node {$areaB$};
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=3.0:5.0] plot(\x,{(-0.5--0.5*\x)/0.5});
}

\newcommand{\areaBp}{
  \fill[line width=2.pt,color=zzwwqq,fill=zzwwqq,fill opacity=0.1] (5.,2.5) -- (3.5,2.5) -- (5.,1.) -- cycle;
  \draw[color=zzwwqq] (4.5,2.) node {$areaB'$};
}
\newcommand{\areaC}{
  \fill[line width=2.pt,color=qqwwtt,fill=qqwwtt,fill opacity=0.25] (1.,4.) -- (5.,4.) -- (3.5,2.5) -- (2.5,2.5) -- cycle;
  \draw[color=qqwwtt] (2.768699664953716,3.536745981551138) node {$areaC$};
}

\newcommand{\areaCp}{
  \fill[line width=2.pt,color=qqzzqq,fill=qqzzqq,fill opacity=0.25] (2.5,2.5) -- (3.5,2.5) -- (5.,1.) -- (1.,1.) -- cycle;
  \draw[color=qqzzqq] (2.9078624650952896,1.2962248992718015) node {$areaC'$};
}

\newcommand{\dashh}{
  \draw [line width=1.pt,dash pattern=on 1pt off 3pt,domain=1.:5.] plot(\x,{(--2.5-0.*\x)/1.});
}

\newcommand{\caseA}{
  \draw [red, dashed] (t2)--(a);
  \draw [red] (t1)--(a);
  \nodelabel{t1}{left}
  \nodelabel{t2}{left}
}

\newcommand{\caseB}{
  \draw [red, dashed] (t6)--(b);
  \draw [red] (t5)--(b);
  \nodelabel{t5}{right}
  \nodelabel{t6}{right}
}

\newcommand{\caseC}{
  \draw [red, dashed] (t4)--(r);
  \draw [red] (t3)--(r);
  \nodelabel{t3}{left}
  \nodelabel{t4}{right}
}

\newcommand{\caseCp}{
  \draw [red, dashed] (t8)--(r');
  \draw [red] (t7)--(r');
  \nodelabel{t8}{left}
  \nodelabel{t7}{right}
}

\newcommand{\drawbg}{
  \clip(1.,1.) rectangle (5.,4.);
  \dashh
  \draw[gray, line width=2pt] (a)--(b);
  \nodelabel{a}{above}
  \nodelabel{b}{below}
  \nodelabel{r}{below}
  \nodelabel{r'}{above}
}

\newcommand{\drawbest}{
  \areaA
  \areaAp
  \areaB
  \areaBp
  \areaC
  \areaCp
  \drawra
  \drawrb
  \drawrpa
  \drawrpb
  \draw[red, dashed] (t1)--(a);
  \draw[red, dashed] (a)--(r);
  \draw[red, dashed] (t5)--(b);
  \draw[red, dashed] (b)--(r);
  \draw[red, dashed] (r)--(c);
  \draw[red, dashed] (c)--(t7);
  \draw[red] (r)--(t3);


  \nodelabel{t1}{left}
  \nodelabel{t5}{right}
  \nodelabel{t3}{left}
  \nodelabel{t7}{right}
}

